The relative Brauer group of $K(1)$-local spectra

Using profinite Galois descent, we compute the Brauer group of the $K(1)$-local category relative to Morava E-theory. At odd primes this group is generated by a cyclic algebra formed using any primitive $(p-1)$st root of unity, but at the prime two is a group of order $32$ with nontrivial extensions; we give explicit descriptions of the generators, and consider their images in the Brauer group of $KO$. Along the way, we compute the relative Brauer group of completed $KO$, using the \'etale locally trivial Brauer group of Antieau, Meier and Stojanoska.

==> extras/glossary.tex <==
\newglossaryentry{Sphere}{
    name=\ensuremath{\bm 1_A},
    description={$A$-local sphere spectrum},
}

\newglossaryentry{E}{
    name=\ensuremath{\E},
    description={Morava E-theory, $E_n = E(\F[p^n], \Gamma_n)$},
}
        
\newglossaryentry{K}{
    name=\ensuremath{\K},
    description={Morava K-theory, $K(n) = E_n/(p, v_1, \dots, v_{n-1})$},
}

\newglossaryentry{G}{
    name=\ensuremath{\G},
    description={Extended Morava stabiliser group $\G_n = \mathbb S_n \rtimes \mathrm{Gal}(\F[p^n]/\F[p]) = \mathrm{Aut}(\Gamma_n, \F[p^n])$},
}

\newglossaryentry{W}{
    name=\ensuremath{\W},
    description={Witt vectors $\W = W(\overline{\F}_p)$},
}

\newglossaryentry{SW}{
    name=\ensuremath{\mathbb{SW}},
    description={Spherical Witt vectors $\mathbb {SW} = W^+(\overline{\F}_p)$},
}

\newglossaryentry{et}{
    name=\ensuremath{\et G},
    description={\'Etale classifying site of a profinite group $G$},
}

\newglossaryentry{proet}{
    name=\ensuremath{\proet G},
    description={Pro\'etale classifying site of a profinite group $G$},
}

\newglossaryentry{mathcal E}{
    name=\ensuremath{\mathcal E},
    description={Pro\'etale Morava E-theory sheaf}
}

\newglossaryentry{Pic}{
    name=\ensuremath{\Pic (-) \,(\Picc(-), \pic(-))},
    description={Picard group (resp. space, spectrum)}
}

\newglossaryentry{Br}{
    name=\ensuremath{\Br (-) \,(\Brr(-), \br(-))},
    description={Brauer group (resp. space, spectrum)}
}

\newglossaryentry{Brrel}{
    name=\ensuremath{\Br (- \mid A )},
    description={Relative Brauer group, $\Br(\bm 1 \mid A) \coloneqq \ker \left(\Br(\bm 1) \to \Br(A) \right)$}
}

\newglossaryentry{Brrrel}{
    name=\ensuremath{\Brr' (- \mid A )},
    description={Relative cohomological Brauer space of a $G$-Galois extension, $\Brr'(\bm 1 \mid A) \coloneqq (B\Picc(A))^{hG}$}
}

\newglossaryentry{Brrnel}{
    name=\ensuremath{\Br_1^0},
    description={Brauer group of $\mathcal Sp_{\K}$ relative to $KU_p$, $\Br_1^0 \coloneqq \Br (\bm 1_\K \mid KU_p )$}
}

\newglossaryentry{nr}{
    name = \ensuremath{R\un},
    description = {Maximal unramified extension of a commutative ring spectrum $R$}
}

\newglossaryentry{Dcg}{
    name=\ensuremath{\mathcal D \cg},
    description={Full subcategory of $\mathcal C$-compact generators in a $\mathcal C$-linear \inftycat{} $\mathcal D$}
}

==> sseq/1midB.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = 1midB]

    \foreach \x in {1,...,15}{                     \class(1-2*\x,2*\x-1)
    \class(-2*\x,2*\x)
    \class(-2*\x,2*\x)
    
    \class(2-2*\x,2*\x-1)
    \class(1-2*\x,2*\x)
    \class(1-2*\x,2*\x)
    \class[gray] (-\x, -1 + \x)} 
    
    \class[rectangle](0,0)
    \class(0,0)
    \class[rectangle](1,0)
    \class(1,0)
    
        
    \foreach \x in {0,...,10} {
        \begin{scope}[xshift = 4*\x]
        \foreach \y in {0,...,20}{
            \class(2 - \y, \y ) }
        \end{scope}}
        
    \class[minimum width = width("3") + 0.5em, "3"](4,0)
    \class[minimum width = width("3") + 0.5em, "3"](12,0)
    \class[minimum width = width("3") + 0.5em, "4"](8,0)
            
    \foreach \x in {1,...,10} {
        \begin{scope}[xshift = 4*\x]
        % \class[circlen = 2](-1, 1)
        \foreach \y in {0,...,20}{
            \class(-1 - \y, \y + 1) }
        \end{scope}}
    
    
    % % %differentials
    % % %red
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,10}{
            \d[red]3(6 + \y, \y)
            }
        \end{scope}
    }
    
    % %blue
        \begin{scope}
        \foreach \y in {0,...,8}{
            \d[red]3(1 + \y, 3 + \y)
            }
        \end{scope}
        \begin{scope}
        \foreach \y in {0,...,3}{
            \d[red]3(-3 + \y, 7 + \y)
            }
        \end{scope}
    % \d[red,dashed]3(-1,4) \replacetarget
    % \d[red,dashed]2(-1,1,2,2)
    % \d[red]2(-1,1)
    \d[red]2(-1,2,1)
    % \d[red,dashed]5(-1,2,2)
    
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,11}{
            \d[red]3(4 + \y, \y)
            }
        \end{scope}
    }
    \begin{scope}
        \foreach \y in {0,...,7}{
            \d[red]3(0 + \y, 4 + \y)
            }
        \end{scope}
    \begin{scope}
        \foreach \y in {0,...,3}{
            \d[red]3(-4 + \y, 8 + \y)
            }
        \end{scope}

    \d[red, dashed]2(-1,0)

    
    % %extensions
    % \structline(0,0)(0,1,1)
    \structline(0,1)(0,2)
\end{sseqdata}


==> sseq/1midKO2.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = Br(1midKO2), class pattern = diagonal]

    \class[minimum width = width("3") + 0.5em,"3"](0,0)
    \class[minimum width = width("3") + 0.5em,"3"](-1,1)
    \class[rectangle](0,1)
    \class(0,1)
    \class[rectangle](1,0)
    \class(1,0)
    \class[minimum width = width("2") + 0.5em,"2"](-1,0)
    \class[minimum width = width("2") + 0.5em,"2"](-2,1)

    \foreach\x in {0,...,3}{
    \begin{scope}[xshift = 8*\x]
        \class(2,0)
        \class(1,1)
        \class(3,0)
        \class(2,1)
    \end{scope}
    }

    \class[minimum width = width("3") + 0.5em, "3"](4,1)
    \class[minimum width = width("4") + 0.5em, "4"](8,1)

    \extension[densely dotted](0,0)(0,1,1)
\end{sseqdata}

==> sseq/BmidE.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = Br(BmidE), class pattern = diagonal]
    \foreach \x in {0,...,1} {
        \class(-\x,\x)
        \class[rectangle](1-\x,\x)
        \class(1-\x,\x)
    }

    \class[minimum width = width("2") + 0.5em,"2"](2,1)
    \class[minimum width = width("2") + 0.5em,"3"](4,1)
    \class[minimum width = width("2") + 0.5em,"2"](6,1)
    \class[minimum width = width("2") + 0.5em,"4"](8,1)
    \class[minimum width = width("2") + 0.5em,"2"](10,1)
    \class[minimum width = width("2") + 0.5em,"3"](12,1)

    \structline (0,0) (0,1,1)
\end{sseqdata}

==> sseq/BrauerKO.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = BrauerKO]
    \foreach \x in {2,...,15}{                         \class(1-\x,\x)}
    
    \foreach \x in {1,...,15}{                     \class(-\x,\x)}
    
    \class(0,0)
    \class(0,1)
    \class(1,0)
    
    % \class[circlen = 2](5,1)
    % \class[circlen = 2](-7,1)
        
    \foreach \x in {0,...,10}{
        \begin{scope}[xshift = 4*\x]
        \foreach \y in {0,...,20}{
            \class(2 - 2*\y, 2*\y + 1) }
        \end{scope}}
            
    \foreach \x in {1,...,10} {
    \class[rectangle](4*\x+1,0)
        \begin{scope}[xshift = 4*\x]
        % \class[circlen = 2](-1, 1)
        \foreach \y in {1,...,20}{
            \class(1 - 2*\y, 2*\y) }
        \end{scope}}
    
    
    % %differentials
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,10}{
            \d[red]3(5 + \y, \y)
            }
        \end{scope}
    }
    
    \begin{scope}
        \foreach \y in {0,...,8}{
            \d[red]3(1 + \y, 4 + \y)
            }
        \end{scope}
        \begin{scope}
        \foreach \y in {0,...,3}{
            \d[red]3(-3 + \y, 8 + \y)
            }
    \end{scope}
        
    \d[red]3(-1,2)
    % \d[red,dashed,]3(0,1)
    % \d[red,dashed]3(-4,7)
    \d[red]2(-1,1)
    \d[red]2(-2,2)
    
    \structline (0,0)(0,1)
    \structline (0,1)(0,3)
\end{sseqdata}


==> sseq/BrauerKO2.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = BrauerKO2, class pattern = diagonal]
    \foreach \x in {1,...,15}{                         \class(1-\x,\x)}
    
    \foreach \x in {1,...,7}{                         \class(1-2*\x, 2*\x)}
    
    \foreach \x in {1,...,15}{                     \class(-\x,\x)}
    
    \class[rectangle](1,0)
    \class(0,0)
    \class(1,0)
    
    % \class[circlen = 2](5,1)
    % \class[circlen = 2](-7,1)
        
    \foreach \x in {0,...,10} {
        \begin{scope}[xshift = 4*\x]
        \foreach \y in {0,...,20}{
            \class(2 - 2*\y, 2*\y + 1) }
        \end{scope}}
            
    \foreach \x in {1,...,10} {
        \begin{scope}[xshift = 4*\x]
        \class[rectangle](1,0)
        % \class[circlen = 2](-1, 1)
        \foreach \y in {1,...,20}{
            \class(1 - 2*\y, 2*\y) }
        \end{scope}}
    
    
    % %differentials
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,10}{
            \d[red]3(5 + \y, \y)
            }
        \end{scope}
    }
    
    \begin{scope}
        \foreach \y in {0,...,8}{
            \d[red]3(1 + \y, 4 + \y)
            }
        \end{scope}
        \begin{scope}
        \foreach \y in {0,...,3}{
            \d[red]3(-3 + \y, 8 + \y)
            }
    \end{scope}
        
    \d[red]3(-1,2,2)
    % \d[red,dashed,]3(0,1)
    % \d[red,dashed]3(-3,4,1)
    \d[red]2(-1,1)
    \d[red]2(-2,2)(-3,4,2)
    
    \structline(-1,2,1)(-1,6)
    \structline (0,0)(0,1)
    \structline (0,1)(0,3)
\end{sseqdata}

==> sseq/BrauerKOp.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = BrauerKOp, class pattern = diagonal]

    \foreach \x in {0,...,10}{          \class(-\x, \x)}
    
    \foreach \x in {1,...,5}{          \class["\times/\times^2", draw = none](1 - 2*\x,2*\x)
    \class["{\times_2}", draw = none](2- 2*\x,-1 + 2*\x)}
    
    \class["\square^\times", draw=none](1,0)
    \class[rectangle](5,0)
    \class[rectangle](9,0)

    \d[red]2 (-1,1)
\end{sseqdata}

==> sseq/BrauerSSeven.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = Brauersseven, no struct lines, class pattern = diagonal]
     
    %CLASSES
    \Ptower(0,0){15}
    \Ptower(-1,1){15}

    \PPLtower(1,0)[rectangle]{15}
    \PPRtower(0,1)[rectangle]{15}
    \Ptower(1,0){15}
    \Ptower(0,1){15}

    \foreach\x in {0,...,10}{
    \begin{scope}[xshift = 4*\x]
        \PPEtower(2,1){15}
    \end{scope}
    }
    
    \PPEtower(4,1)[minimum width = width("3") + 0.5em, "3"]{15}
    \PPEtower(8,1)[minimum width = width("4") + 0.5em, "4"]{15}
    \PPEtower(12,1)[minimum width = width("3") + 0.5em, "3"]{15}
    \PPEtower(16,1)[minimum width = width("5") + 0.5em, "5"]{15}
    \PPEtower(20,1)[minimum width = width("3") + 0.5em, "3"]{15}
    \PPEtower(24,1)[minimum width = width("4") + 0.5em, "4"]{15}
    \PPEtower(28,1)[minimum width = width("3") + 0.5em, "3"]{15}
    \PPEtower(32,1)[minimum width = width("6") + 0.5em, "6"]{15}
    \PPEtower(36,1)[minimum width = width("3") + 0.5em, "3"]{15}

    \structline[green](0,0)(-1,1,2)
    \structline[green](1,0,1)(0,1,1)
    \structline[green](1,0,2)(0,1,3)
    \structline[green](-1,2,1)(-2,3,1)


    %STRUCTULINES
    \foreach\y in {1,...,14}{
    \structline[green](-\y, \y,1)(-1-\y,1+ \y,2)
    \structline[green](1-\y, \y,2)(-\y,1+ \y,3)
    }
    
    %DIFFERENTIALS
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,10}{
            \d[red]3(6 + \y, 1 + \y)
            }
        \end{scope}
    }
    
        \begin{scope}
        \foreach \y in {0,...,8}{
            \d[red]3(1 + \y, 4 + \y)
            }
        \end{scope}
        \begin{scope}
        \foreach \y in {0,...,3}{
            \d[red]3(-3 + \y, 8 + \y)
            }
        \end{scope}
    
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,11}{
            \d[red]3(4 + \y, 1 + \y)
            }
        \end{scope}
    }
    \begin{scope}
        \foreach \y in {0,...,7}{
            \d[red]3(0 + \y, 5 + \y)
            }
        \end{scope}
    \begin{scope}
        \foreach \y in {0,...,3}{
            \d[red]3(-4 + \y, 9 + \y)
            }
        \end{scope}

    \d[red]2(-1,1)(-2,3,2)
    \d[red]3(-1,2,2)
    % \d[red,dashed]5(-1,2,3)
    % \replacesource[red]

    \classoptions["{q_1}"{above right={.1pt}}](-1,1,2)
    \classoptions["{q_2}"{below={.2pt}}](-1,2,1)
    \classoptions["{q_2'}"{above right={.1pt}}](-1,2,3)
    \classoptions["{q_4}"{above right={.1pt}}](-1,4)
    \classoptions["{q_6}"{above right={.1pt}}](-1,6)
    \classoptions["{1 + \varepsilon}"{above={1pt}}](1,2)

    %EXTENSIONS
    \extension(0,0)(0,1,1)
    \extension(0,1,2)(0,3)
    \extension[bend left = 5](-1,2,1)(-1,6)
    \extension(-1,1,2)(-1,2,3)
    \extension(-1,2,3)(-1,4)
\end{sseqdata}


==> sseq/PicardSSOdd.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = PicardSSOdd]
    \foreach \x in {0,...,5} {
        \class(-\x,\x)
        \class["\times", draw=none](-1-\x,2+\x)
    }
    \foreach \x in {0,...,1} {
        \class["\square^\times", draw=none](1-\x,\x)
    }
    % \class(2,1)
    % \class(4,1)
    \class[minimum width = width("2") + 0.5em,"1"](4,1)
    \class[minimum width = width("2") + 0.5em,"1"](8,1)
    \class[minimum width = width("2") + 0.5em,"2"](12,1)
    % \class(8,1)
    % \class(10,1)

    \d[red]2 (-1,1)
\end{sseqdata}

==> sseq/scrap/Steenrod.tex <==
\begin{sseqdata}[Adams grading, name = Steenrod, classes = {draw = none}]
    \foreach \y in {0,...,2}{
        \class["0_{\y}"](0,\y)
        \class["1_{\y}"](-1,\y)
        \class["2_{\y}"](-2,\y)
        \class["3_{\y}"](-3,\y)
        \class["21_{\y}"](-3,\y)
        \class["31_{\y}"](-4,\y)
        \class["4_{\y}"](-4,\y)
    }
    
    \d[red]2(0,0)
    \d[red]1(-2,1)
    \d[red]1(-3,1,2)(-4,2,1)
    \d[red]1(-3,0,2)
    \d[red]1(-2,0)


    \structline (0,1)(0,2)
    \structline (-1,0)(-1,1)
    
\end{sseqdata}

==> sseq/scrap/eqSteenrod.tex <==
\begin{sseqdata}[Adams grading, name = eqSteenrod4]
    \foreach \x in {0,...,10}{
        \class(-\x,\x)
        \class(-1-\x,\x)
        \class(-2-\x,\x)
        \class(-3-\x,\x)
        \class(-3-\x,\x)
        \class[draw = none, "*"](-4-\x,\x)
        \class[draw = none, "*"](-5-\x,\x)
        \class[draw = none, "*"](-6-\x,\x)
    }
    \foreach \x in {0,...,3}{
        \structline[red] (-1-2*\x,1+2*\x)(-2*\x-2,2*\x+2)
        \structline[red] (-2-2*\x,1+2*\x)(-3-2*\x,2*\x+2)
        \structline[red] (-2-2*\x,2*\x)(-3-2*\x,2*\x+1)
        \structline[red] (-3-2*\x,2*\x,1)(-4-2*\x,2*\x+1,1)
        \structline[red] (-3-2*\x,2*\x,2)(-4-2*\x,2*\x+1,2)

        \structline[blue, bend left = 20] (-2*\x,2*\x)(-2-2*\x,2*\x+2)
        \structline[blue, bend left = 20] (-1-2*\x,2*\x)(-3-2*\x,2*\x+2)
        \structline[blue, bend left = 20] (-2-2*\x,2*\x)(-4-2*\x,2*\x+2)
        \structline[blue, bend left = 20] (-3-2*\x,2*\x,1)(-5-2*\x,2*\x+2,1)
        \structline[blue, bend left = 20] (-3-2*\x,2*\x,2)(-5-2*\x,2*\x+2,2)

        \structline[blue, bend right = 20] (-1-2*\x,1+2*\x)(-1-2-2*\x,1+2*\x+2)
        \structline[blue, bend right = 20] (-1-1-2*\x,1+2*\x)(-1-3-2*\x,1+2*\x+2)
        \structline[blue, bend right = 20] (-1-3-2*\x,1+2*\x,1)(-1-5-2*\x,1+2*\x+2,1)
        \structline[blue, bend right = 20] (-1-2-2*\x,1+2*\x)(-1-4-2*\x,1+2*\x+2)
        \structline[blue, bend right = 20] (-1-3-2*\x,1+2*\x,2)(-1-5-2*\x,1+2*\x+2,2)
    }
    
    % \foreach \x in {0,...,3}{
    %     \structline[red, bend left = 20] (-\x,\x)(-2-\x,\x+2)
    %     \structline[red, bend left = 20] (-1-\x,\x)(-3-\x,\x+2)
    %     \structline[red, bend left = 20] (-2-\x,\x)(-4-\x,\x+2)
    %     \structline[red, bend left = 20] (-3-\x,\x,1)(-5-\x,\x+2,1)
    %     \structline[red, bend left = 20] (-3-\x,\x,2)(-5-\x,\x+2,2)
    % }

\end{sseqdata}

\begin{sseqdata}[Adams grading, name = eqSteenrod8]
    \foreach \x in {0,...,10}{
        \class(-\x,\x)
        \class(-1-\x,\x)
        \class(-2-\x,\x)
        \class(-3-\x,\x)
        \class(-3-\x,\x)
        \class[draw = none, "*"](-4-\x,\x)
        \class[draw = none, "*"](-5-\x,\x)
        \class[draw = none, "*"](-6-\x,\x)
    }
    \foreach \x in {0,...,3}{
        \structline[green] (-2*\x,2*\x)(-2*\x-1,2*\x+1)
        \structline[green] (-1-2*\x,2*\x)(-2-2*\x,2*\x+1)
        \structline[green] (-2-2*\x,2*\x)(-3-2*\x,2*\x+1)
        \structline[green] (-3-2*\x,2*\x,1)(-4-2*\x,2*\x+1,1)
        \structline[green] (-3-2*\x,2*\x,2)(-4-2*\x,2*\x+1,2)

        \structline[orange, bend left = 20] (-2*\x,2*\x)(-2-2*\x,2*\x+2)
        \structline[orange, bend left = 20] (-1-2*\x,2*\x)(-3-2*\x,2*\x+2)
        \structline[orange, bend left = 20] (-2-2*\x,2*\x)(-4-2*\x,2*\x+2)
        \structline[orange, bend left = 20] (-3-2*\x,2*\x,1)(-5-2*\x,2*\x+2,1)
        \structline[orange, bend left = 20] (-3-2*\x,2*\x,2)(-5-2*\x,2*\x+2,2)

        \structline[orange, bend right = 20] (-1-2*\x,1+2*\x)(-1-2-2*\x,1+2*\x+2)
        \structline[orange, bend right = 20] (-1-1-2*\x,1+2*\x)(-1-3-2*\x,1+2*\x+2)
        \structline[orange, bend right = 20] (-1-3-2*\x,1+2*\x,1)(-1-5-2*\x,1+2*\x+2,1)
        \structline[orange, bend right = 20] (-1-2-2*\x,1+2*\x)(-1-4-2*\x,1+2*\x+2)
        \structline[orange, bend right = 20] (-1-3-2*\x,1+2*\x,2)(-1-5-2*\x,1+2*\x+2,2)
    }
    
    % \foreach \x in {0,...,3}{
    %     \structline[green, bend left = 20] (-\x,\x)(-2-\x,\x+2)
    %     \structline[green, bend left = 20] (-1-\x,\x)(-3-\x,\x+2)
    %     \structline[green, bend left = 20] (-2-\x,\x)(-4-\x,\x+2)
    %     \structline[green, bend left = 20] (-3-\x,\x,1)(-5-\x,\x+2,1)
    %     \structline[green, bend left = 20] (-3-\x,\x,2)(-5-\x,\x+2,2)
    % }

\end{sseqdata}

==> sseq/scrap/obstructionKO2.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = obstructionKO2]

    \class["{H^1}", draw = none](0,1)
    \class["{H^0}", draw = none](1,0)
    
    % \class[circlen = 2](5,1)
    % \class[circlen = 2](-7,1)
        
    \foreach \x in {0,...,10} {
        \begin{scope}[xshift = 4*\x]
        \foreach \y in {1,...,20}{
            \class(3 - 2*\y, 2*\y ) }
        \end{scope}}
            
    \foreach \x in {1,...,10} {
        \begin{scope}[xshift = 4*\x]
        \foreach \y in {1,...,20}{
            \class(2 - 2*\y,-1 + 2*\y) }
        \end{scope}}

  
    \foreach \y in {1,...,20}{
            \class[draw = none, "{*}"](2*\y + 1,0)}
    
    
    %differentials
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {2,...,10}{
            \d[red]3(6 + \y, -1 + \y)
            }
        \end{scope}
    }
    
    \begin{scope}
        \foreach \y in {0,...,8}{
            \d[red]3(2 + \y, 3 + \y)
            }
        \end{scope}
        \begin{scope}
        \foreach \y in {0,...,3}{
            \d[red]3(-2 + \y, 7 + \y)
            }
    \end{scope}

\end{sseqdata}

==> sseq/scrap/obstructiondetKO2.tex <==
\begin{sseqdata}[Adams grading, scale = .8, name = obstructiondetKO2]
        
    % \foreach \x in {0,...,10} {
    %     \begin{scope}[xshift = 4*\x]
    %     \foreach \y in {0,...,20}{
           
    %     \end{scope}}
        
            
    \foreach \x in {0,...,20} {
        \begin{scope}[xshift = 2*\x]
            \class["{*}", draw = none](2,0)
        \foreach \y in {0,...,20}{
            \class(1 - \y, \y + 1)}
        \end{scope}}

    \class["{H^1}", draw = none](0,1)
    \class["{H^0}", draw = none](1,0)
    
    % % %differentials
    % % %red
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,10}{
            \d[red]3(7 + \y, 1 + \y)
            }
        \end{scope}
    }
    
    % % %blue
        \begin{scope}
        \foreach \y in {0,...,8}{
            \d[red]3(2 + \y, 2 + \y)
            }
        \end{scope}
        \begin{scope}
        \foreach \y in {1,...,3}{
            \d[red]3(-2 + \y, 6 + \y)
            }
        \end{scope}
    
    \foreach \x in {0,...,1} {
        \begin{scope}[xshift = 8*\x]
        \foreach \y in {0,...,11}{
            \d[red]3(9 + \y, 1 + \y)
            }
        \end{scope}
    }
    \begin{scope}
        \foreach \y in {0,...,7}{
            \d[red]3(1 + \y, 3 + \y)
            }
        \end{scope}
    \begin{scope}
        \foreach \y in {1,...,4}{
            \d[red]3(-3 + \y, 7 + \y)
            }
        \end{scope}
    \d[red, dashed]3(-2,6)
    \d[red, dashed]3(-3,7)
    
    % % %extensions
    % % \structline(0,0)(0,1,1)
    % \structline(0,1)(0,2)
\end{sseqdata}


==> zstyle/preamble.tex <==
\usepackage{zstyle/main}
\RequirePackage{quiver}
\addbibresource{extras/references.bib}

\usepackage[normalem]{ulem} %strikeout


\def\Prsm{\mathrm{Pr}^{L, \mathrm{smon}}}
\def\Pic{\mathrm{Pic}}
\def\pic{\mathfrak{pic}}
\def\Picc{\mathfrak{Pic}}
\def\Br{\mathrm{Br}}
\def\LBr{\mathrm{LBr}}
\def\br{\mathrm{br}}
\def\Brr{\mathfrak{Br}}
\def\Az{\mathrm{Az}}
\def\az{\mathrm{az}}
\def\Azz{\mathfrak{Az}}
\def\E{\mathbf E}
\def\K{\mathbf K}
\def\G{\mathbb G}
\def\Sq{\mathrm{Sq}}
\def\GL{\mathrm{GL}}
\def\PGL{\mathrm{PGL}}
\def\gl{\mathfrak{gl}}
\def\cg{^{\mathrm{ecg}}}
\def\un{^{\mathrm{nr}}}
\def\eMap{\underline{\smash{\mathrm{Map}}}}
\def\eEnd{\underline{\smash{\mathrm{End}}}}
\def\eFun{\underline{\smash{\mathrm{Fun}}}}
\def\Spet{\operatorname{Spec}}
\def\cd{\operatorname{cd}}
\newcommand{\proet}[1]{B{#1}_{\operatorname{pro\acute{e}t}}}
\newcommand{\et}[1]{B{#1}_{\operatorname{\acute{e}t}}}
\SseqNewClassPattern{diagonal}{
    (0,0);
    (-0.1,-0.1)(0.1,0.1);
    (-0.2,-0.2)(0,0)(0.2,0.2);
}
\def\Rig{\mathrm{Rig}}
\def\CRig{\mathrm{CRig}}
\def\Mon{\mathrm{Mon}}
\def\CMon{\mathrm{CMon}}
\def\grp{^{\mathrm{gp}}}
\def\BMod{\mathrm{BMod}}
\def\Sh{\mathrm{Sh}}

%listofsymbols
\loadglsentries{extras/Glossary}


%SPECTRAL SEQUENCES TOWERS
%Polynomial towers with generator in degree 1. The optional argument describes the bottom class
\DeclareSseqGroup\Ptower{om}{
    \class[#1](0,0)
    \foreach\y in {1,...,#2}{
    \class(-\y, \y)
    \structline[blue]
    }
}

%Polynomial towers with generator in degree 2. The optional argument describes the bottom class
\DeclareSseqGroup\PPtower{om}{
    \class[#1](0,0)
    \foreach\y in {1,...,#2}{
    \class(-2*\y, 2*\y)
    \structline[orange]
    }
}

%Polynomial towers with generator in degree 2 (multiplications on left). The optional argument describes the bottom class
\DeclareSseqGroup\PPLtower{om}{
    \class[#1](0,0)
    \foreach\y in {1,...,#2}{
    \class(-2*\y, 2*\y)
    \structline[orange, bend right = 10]
    }
}

%Polynomial towers with generator in degree 2 (multiplications on left). The optional argument describes the bottom class
\DeclareSseqGroup\PPRtower{om}{
    \class[#1](0,0)
    \foreach\y in {1,...,#2}{
    \class(-2*\y, 2*\y)
    \structline[orange, bend left = 10]
    }
}

%Towers with polynomial generator in degree 2 and exterior generator in degree 1. The optional argument describes the bottom class. Bracketed argument gives page range for structlines
\DeclareSseqGroup\PPEtower{omo}{
    \class[#1](0,0)
    \foreach\y in {0,...,#2}{
    \begin{scope}[xshift = -2*\y, yshift = 2*\y]
        \class(-1,1)
        \structline[blue]
        % \structlineoptions[page = #3]
        \class(-2,2)
    \end{scope}
    }
    \class(-3-2*#2, 3 + 2*#2)

    \foreach\y in {0,...,#2}{
    \structline[orange, bend right = 10](-2*\y,2*\y)(-2*\y-2,2*\y+2)
    % \structlineoptions[page = #3]
    
    \structline[orange, bend left = 10](-1-2*\y,1+2*\y)(-2*\y-3,2*\y+3)
    % \structlineoptions[page = #3]
    }
}



\input{sseq/1midB}
\input{sseq/BmidE}
\input{sseq/BrauerKO2}
\input{sseq/BrauerKO}
\input{sseq/BrauerSSeven}
\input{sseq/PicardSSOdd}
\input{sseq/1midKO2}
\input{sseq/BrauerKOp}




\title{The relative Brauer group of \texorpdfstring{$K(1)$}{K(1)}-local spectra}
\author{Itamar Mor}
% \date{DRAFT - \today}


\setcounter{tocdepth}{2}



